Range, not Independence, Drives Modularity in Biologically Inspired Representations

Why do biological and artificial neurons sometimes modularise, each encoding a single meaningful variable, and sometimes entangle their representation of many variables? In this work, we develop a theory of when biologically inspired networks -- those that are nonnegative and energy efficient -- modularise their representation of source variables (sources). We derive necessary and sufficient conditions on a sample of sources that determine whether the neurons in an optimal biologically-inspired linear autoencoder modularise. Our theory applies to any dataset, extending far beyond the case of statistical independence studied in previous work. Rather we show that sources modularise if their support is ``sufficiently spread''. From this theory, we extract and validate predictions in a variety of empirical studies on how data distribution affects modularisation in nonlinear feedforward and recurrent neural networks trained on supervised and unsupervised tasks. Furthermore, we apply these ideas to neuroscience data, showing that range independence can be used to understand the mixing or modularising of spatial and reward information in entorhinal recordings in seemingly conflicting experiments. Further, we use these results to suggest alternate origins of mixed-selectivity, beyond the predominant theory of flexible nonlinear classification. In sum, our theory prescribes precise conditions on when neural activities modularise, providing tools for inducing and elucidating modular representations in brains and machines.

==> Old_Writing/Scrap_Maths.tex <==
\subsection{Optimal Nonlinear Representations are sometimes just Linear}\label{sec:opt_nonlinear_rep_linear}

Let's consider a slightly different setting. The representation can be any positive nonlinear function of the variables, but still has to be linearly readout:
\begin{equation}
    \mR \vg(t) + \vb_R= \begin{bmatrix}
        x(t) \\ y(t)
    \end{bmatrix}
\end{equation}
When is the optimal representation still just a linear function of both variables and a bias:
\begin{equation}
    \vg(t) = \vu x(t) + \vv y(t) + \vb
\end{equation}
It is intuitive that the representation must contain at least these components. The linear components must be included so that they can be linearly readout, and something like the bias must be included to make the representation positive. Nonlinear functions of $x(t)$ or $y(t)$ (or both) could be included, but, as we'll show they don't help the readout and they cost in activity. So, they are only added if they help you achieve positivity at a cheaper energy cost than adding a constant offset.

We'll begin with a simpler one variable representation. Imagine you wanted to add a nonlinear component to a representation of $x(t)$:
\begin{equation}
    \vg(t) = \vu x(t) + \vw f(x(t)) + \vb
\end{equation}
We can expand this nonlinearity in an orthogonal polynomial basis defined with respect to the probability distribution on $x(t)$ as $t$ varies between $1$ and $T$: $f(x(t)) = f_0 + f_1 x(t)+ \sum_i f_i H_i(x(t))$, with the property that:
\begin{equation}
    \langle H_i(x(t))H_j(x(t))\rangle_t = \delta_{ij} \quad \langle H_i(x(t))\rangle_t = 0 \quad \langle H_i(x(t)) x(t)\rangle_t = 0
\end{equation}
Without loss of generality we can set $f_0$ and $f_1$ to zero by absorbing their contribution into the constant and linear terms, $\vb$ and $\vu x(t)$. 

First, we'll show that having this nonlinear component never decreases the readout loss $|\mR|^2_F$. In this example of a representation encoding only a single variable the vector forming $\mR$ must be orthogonal to all components of the representation that aren't either linear or constant:
\begin{equation}
    \mR\cdot\vg(t) +\vc = \underbrace{\mR\vu x(t)}_{\text{Linear}} + \underbrace{\mR\vb + \vc}_{\text{Constant}} + \underbrace{\mR\vw f(x(t))}_{\text{Nonlinear}} = x(t)
\end{equation}
If $\vu$ and $\vw$ are orthogonal $\mR$ is not changed by including the nonlinear component, else the length of the vector $\mR$, and hence the weight loss, must increase to ensure that both $\mR\vu = 1$ and $\mR\vw = 0$ (fig). So the readout loss is at best ambivalent about including a nonlinear component in the representation.

Second, including the nonlinear component will only increase the activity loss:
\begin{equation}
\begin{split}
        \langle|\vg(t)|^2\rangle_t = \langle |\vu x(t) + \vb|^2\rangle_t + |\vw|^2\langle f(x(t))^2\rangle_t  + 2\vw\cdot\vu\langle x(t)f(x(t))\rangle_t  + 2\vw \cdot \vb \langle f(x(t))\rangle_t \\
        = \langle |\vu x(t) + \vb|^2\rangle_t + |\vw|^2\langle f(x(t))^2\rangle_t  + \sum_i \bigg[2f_i\vw\cdot\vu\langle x(t)H_i(x(t))\rangle_t  + 2f_i\vw \cdot \vb \langle H_i(x(t))\rangle_t\bigg] \\        = \langle |\vu x(t) + \vb|^2\rangle_t + |\vw|^2\langle f(x(t))^2\rangle_t
        \geq \langle |\vu x(t) + \vb|^2\rangle_t
\end{split}
\end{equation}
Where the third equality follows from the orthogonality properties of these functions $H_i(x)$.

So non-linear components are only added when they can help make it positive at less cost than adding a bias. 

\will{Let's try and work out the conditions when the nonlinear function is better than a bias.}



%We then use the following inequality for the frobenius norm of the product of two matrices \citep{fang1994inequalities}:
%\begin{equation}
%    \sigma_{\min}(\mE)|\mF|_F^2 \leq |\mF\mE|_F^2 \leq \sigma_{\max}(\mE)|\mF|_F^2
%\end{equation}
%where $\sigma_{\min}(\mE)$ is the minimal singular value of $\mE$. Since both singular values of both the rotation matrices are 1, they therefore have no effect on the frobenius norms in the last line of equation~\ref{eq:recurrent_weight_frob_development}, hence:
%\begin{equation}
%    |\mW|_F^2 = \Tr[\vd_{11}\mD_{11}] + \Tr[\vd_{22}\mD_{22}] = \sum_{i=1}^2 |\va_i|^2|\mA_i|^2 + \underbrace{2\va_i^T\vb_i\mA_i^T\mB_i}_{\text{cross-term}} + |\vb_i|^2|\mB_i|^2
%\end{equation}

For a given length of each coefficient vector, the norms of both readout and recurrent min-norm weight matrices are minimised if the coefficient vectors are orthogonal. For the readout matrix this can be shown using an identical argument to that already developed in section~\ref{sec:weight_loss}. Here we will show that this is also true for the recurrent weight loss:
\begin{equation}\label{eq:recurrent_weight_frob_development}
\begin{split}
    |\mW|_F^2 = \Tr[\mW\mW^T] \\
    = \Tr\Bigg[\begin{bmatrix}
        \va^T_1 \\ \vb_1^T \\ \va_2^T \\ \vb_2^T
    \end{bmatrix}\begin{bmatrix}
        \va_1 & \vb_1 & \va_2 & \vb_2
    \end{bmatrix}\begin{bmatrix}
        \mR_1 & 0 \\
        0 & \mR_2
    \end{bmatrix}\begin{bmatrix}
        \mA_1^T \\ \mB_1^T \\ \mA_2^T \\ \mB_2^T
    \end{bmatrix}\begin{bmatrix}
        \mA_1 & \mB_1 & \mA_2 & \mB_2
    \end{bmatrix} \begin{bmatrix}
        \mR_1^T & 0 \\
        0 & \mR_2^T
    \end{bmatrix}\Bigg]\\
    = \Tr\Bigg[\begin{bmatrix}
        \vd_{11} & \vd_{12} \\
        \vd_{12}^T & \vd_{22}
    \end{bmatrix}\begin{bmatrix}
        \mR_1 & 0 \\
        0 & \mR_2
    \end{bmatrix}\begin{bmatrix}
        \mD_{11} & \mD_{12} \\
        \mD_{12}^T & \mD_{22}
    \end{bmatrix}\begin{bmatrix}
        \mR^T_1 & 0 \\
        0 & \mR^T_2
    \end{bmatrix} \Bigg] \\= \Tr[\vd_{11}\mR_1\mD_{11}\mR_1^T] + \Tr[\vd_{22}\mR_2\mD_{22}\mR_1^T]
\end{split}
\end{equation}
Where we have introduced matrices such as:
\begin{equation}
    \vd_{12} = \begin{bmatrix}
        \va_1^T\va_2 & \va_1^T\vb_2 \\
        \vb_1^T\va_2 & \vb_1^T\vb_2
    \end{bmatrix}
\end{equation}
And equivalent definitions for $\vd_{11}$ or for the capitalised set of vectors. 


==> Old_Writing/Scrap_Text.tex <==
% % v1
% Biological neurons are sometimes precisely modularised, encoding a single meaningful variable, at other times confusingly mixed. Neuroscientists would like to understand when and why such we should expect our discrete categorisations of the world to be recreated in the modularisation of neural hardware. Similarly, machine learners are hopeful of building and understanding disentangled representations. Here, we study optimal representations constrained by biological positivity and energy efficiency. We mathematically show precise conditions on task structure that lead to modularisation of function in linear and partially non-linear settings. Specifically, we show that modularisation is often driven by range-independence  properties (when knowing the value of one variable doesn’t constrain the range of others), rather than statistical independence. We use these conditions to understand and predict tasks in which optimal networks should modularise, and those in which they shouldn’t, and show the effectiveness of these ideas across tasks and architectures. Further, we apply these ideas to neuroscience. In prefrontal cortex we use it to explain why some experiments find cleanly orthogonal encoding of different memories, and others mixed codes. Finally, we show how there could be clean modular neurons in entorhinal cortex that are mistaken as mixed-selective by our current analysis techniques. This work gives precise mathematical constraints on when neural responses should modularise, providing tools for understanding modularity patterns in brains and machines.

Why are things sometimes modular and sometimes not? (neurons interpretable and sometimes not?) Interesting question for neuroscience and ML.

Lots of people have said modularity of some sort is a necessary part of being clever, or have tried to build modularity into networks to make them clever. Here are some existing stories about why neurons might sometimes end up being modular:
\begin{enumerate}
    \item \citet{yang2019task} and \citet{driscoll2022flexible}: RNNs trained on many tasks with shared components learn neural modules that perform sensible computations, e.g. the shared component among the tasks.
    \item \citet{saxe2022neural}: the learning dynamics can lead to the breaking of the network into parts in order of when they are learnt. 
    \item \citet{jarvis2023specialization}: show a surprising case of clear modular structure that simple linear networks never learn.
    \item \cite{shi2022learning} show that deep multipathway networks learn different parts of the problemm. 
    \item \citet{schug2024discovering}: show conditions in a compositional linear hypernetwork teacher-student settings for the student to recover the teacher's compositional structure.
    \item \citet{whittington2022disentanglement}: with regularisation representations of independent variables that are being read out to orthogonal readouts should be in different neurons.
    \item Disentangling world has explored constraints to things modularise in representation, MANY, most related are similar-ish constraints in \citet{hsu2024disentanglement, hsu2024tripod}, or range independence funkiness in \citet{roth2023disentanglement}
\end{enumerate}
\will{Any to add?}

Here we present another story about when things modularise in linear-ish networks. Extends \citep{whittington2022disentanglement} to a lot of dependent data. This idea might generalise to some cool nonlinear things (?), could be useful for ML people into disentangling (???), and could help us understand some funky neural data (??). 

\section{Feedforward Linear Functions}

Our setting: positive linear autoencoder, regularise the activity and the readout weights.

Our result: very specific set of settings in which you get the formation of perfect modules, and we can describe this setting. See fig for sketch of this setting, and then see same fig for evidence of this in simple 2D data. Perhaps emphasise that this includes highly dependent, even heavily linearly correlated, data being modularised, with fig to show this. Try and come up with the best sketch presentation of the maths.

\section{Non-Orthogonal Readouts}

Thus far the variables that we have been hoping to modularise and the ones that are being orthogonally decoded have been synonymous. We will now consider the case where they are decoded to non-orthogonal output channels, for example, for 2 variables:
\begin{equation}
    \mR \vg(t) = \begin{bmatrix}
        x(t) + \cos(\phi) y(t) \\ \sin(\phi) y(t)
    \end{bmatrix}
\end{equation}
This requires us to re-study the weight loss. For the following representation:
\begin{equation}
    \vg(t) = \vu x(t) + \vv y(t) + \vb 
\end{equation}
We can write the readout matrix as
\begin{equation}
    \mR = \begin{bmatrix}
        1 & \cos(\phi) \\
        0 & \sin(\phi)
    \end{bmatrix}\begin{bmatrix}
        \vu_\perp^T \\
        \vv_\perp^T
    \end{bmatrix}
    \end{equation}
Using the same vectors $\vu_\perp$ and $\vv_\perp$ as in section~\ref{sec:weight_loss}. Calling $\theta$ the angle between $\vu$ and $\vv$, we can derive the loss as:
\begin{equation}
\begin{split}
    |\mR|_F^2 = \Tr[\mR\mR^T] = |\vu_\perp|^2 + 2\cos(\phi)\vu_\perp ^T\vv_\perp + \sin^2(\phi)|\vv_\perp|^2 \\
    = \frac{1}{\sin^2(\theta)}\bigg(\frac{1}{|\vu|^2} - \frac{2\cos(\phi)\cos(\theta)}{|\vu||\vv|}+ \frac{\sin^2(\phi)}{|\vv|^2} \bigg)
\end{split}
\end{equation}
In general, for a given $|\vu|$ and $|\vv|$ and $\phi \neq \frac{\pi}{2}$, the optimal alignment will not be orthogonal, i.e. $\theta \neq \frac{\pi}{2}$. This means modularising the code, in which the alignment is $\theta = \frac{\pi}{2}$, is necessarily costly. We therefore have to answer a slightly harder question than before: when does deviating from modular solution decrease the weight loss more than it increases the activity loss?

\will{Getting difficult... To explore: go to modular solution and look and when gradient is away from it, first order effects.}

\will{A semi-bullshit argument: Either the activity loss is minimised at orthogonal, then a small mixing will to first order have no effect on the activity loss, or it is not, then it doesn't want to be modularised. We know to first order the weight loss will have an effect, so it neccesarily will prefer a little bit of mixing?}

\subsection{Other Thoughts}

There's a couple of things it would be really nice to work out:
\begin{itemize}
    \item \sout{Given a target that must be affinely readout, what components should you add, beyond the target itself and a constant offset. You should only add them if they help with achieving positivity at a lower activity cost. This is the same as the constraints we had before.} Done! See above.
    \item Once you have this, you can see if they tend to satisfy the constriants required for modularising? Like, define $x$ and $y$ as the things being linearly readout, then look for the optimal nonlinear representation of them, then look for conditions on the $x$ and $y$ for those nonlinear things to modularise. We actually already have that last part, so what I'm saying is that once we solve the point above, we can say something pretty interesting.
    \item Further, solving the first point would answer the comment I made in the positive linear recurrent neural network section.
    \item We have one last tie to linearity that we need, the readout and weight loss. In the grid cell paper we drop this just by saying: 'ah, push the representation of pairs of things apart'. Can we bake some sense of modularity into this (perhaps into how important it is to separate the representation of different pairs of points) and show, given this assumption, when some interesting things modularise?
    \item Could explore dropping range independence and looking for any weaker condition that means the mixed functional encodings are worse than the univariate ones, and therefore you don't get that happening.
\end{itemize}


\section{Miscellaneous}

\will{Some thoughts to add somewhere:
\begin{itemize}
    \item That extreme point independence might only emerge after a very long time, that what matters is what happens in the relevant time window.
\end{itemize}}


\subsubsection{Modularising out a Single Variable from a Multivariate Representation}

\will{This section is wrong. It compares all mixed solutions to a particular modular solution. In reality we need to compare to the best modular solution. This is hard to calculate.}

A more precise question we can ask is when does a multivariate representation modularise out one variable from all the others? Assuming range symmetry, consider the mixed single-neuron representation of $x$ and a set of $M$ variables $y_i(t)$:
\begin{equation}
    g(t) = x(t) + \sum_{i=1}^M w_i y_i(t) + b_x + b_z - \Delta = x(t) + z(t) + b_x + b_z - \Delta
\end{equation}
Where we have dropped the coefficient beside $x(t)$ by, without loss of generality, setting it to 1. This is allowed as both the modular and the mixed activity loss scale the same way when you multiply the representation by a scalar, so doing so won't change our modularity result, and we can use that degree of freedom to set the coefficient of $x$ to 1.

We can then check, for each choice of coefficient vector $\vw$, whether the mixed solution is preferred over an ideal modular solution

\will{Nope this method ain't gonna work. The weight loss might be different between the perfect modular solution and the proposed one, in a way that stops the solution from modularising...}

This is now very similar to our previous analysis, we know it is optimal to modularise $x$ and $z$ when:
\begin{equation}\label{eq:multivariate_peeling_inequality}
    \Delta < b_x - \sqrt{b_x^2 + b_z^2  - 2\langle x(t)z(t)\rangle_t}
\end{equation}
But now this is again a set of many conditions that depend on the coefficient vector $\vw$. This is saying that if you can find any linear combination of other variables that satisfy the standard 2D corner cutting requirements then you shouldn't modularise. If not, you should modularise. This also provides an iterative alternative route to the complete modularisation route of the previous section: choose a variable, check if this property holds when compared to a linear combination of all the other variables, if so it modularises out. Repeat until you run out of variables or the condition is broken. Again, if the variables are not symmetric around zero then everytime the solution you are considering involves flipping the variable from its prefered orientation you add an offset to the critical delta value equal to $w_i^2(y_{i,\max}^2 - b_i^2)$, as in section~\ref{sec:range_assymmetry}.

\will{Is there any way this is like 'non-commutative'? The whole thing might modularise but the peeling off thing won't?}

\will{Should really show the weight loss property for this setting too, not very hard...}

\subsubsection{Modularisation of Multidimensional Variables}

\will{This section is also wrong for similar reasons. We need to compare to the best case scenario, and that means the }

Perhaps a more useful multivariate case than asking when all of a particular set of variables will modularise from one another is asking when two sets of variables will modularise, or equivalently, when two particular multi-dimensional variables will modularise. Let's consider a mixed single neuron representation of two vector variables $\vx(t)$ and $\vy(t)$:
\begin{equation}
    g = \vu^T\vx + \vv^T\vy + \vu^T\vb_x + \vv^T\vb_y - \Delta
\end{equation}
The modularity condition then becomes:
\begin{equation}\label{eq:multivariate_module_inequality}
    \Delta \leq \vu^T\vb_x + \vv^T\vb_y - \sqrt{ (\vu^T\vb_x)^2 + (\vv^T\vb_y)^2 - 2\vu^T\langle \vx(t)\vy(t)\rangle \vv}
\end{equation}
Again, if the variables are not range symmetric you introduce the appropriate direction flipping penalities introduced in section~\ref{sec:range_assymmetry}. This is saying that the variables group-modularise when there is no linear combination of the two sets of variables which produces a plane with the same corners missing as in the original two variable case. Further, the equivalent of the extreme point independent property that holds no matter the correlation structure of the variables is that all linear combinations of the two sets of variables are extreme point independent. This is equivalent to saying that all variables in one group are extreme point independent of all variables in the other group, and vice verse. Notably, this allows variables within the same group to be extreme point dependent. These results can be easily extended to many multivariate variables.

\will{Should really show the weight loss property for this setting too too}


\subsection{Optimal Modular Nonlinear Representations}

Now let's drop the linearity assumption in the representation and show that statistical independence is still enough to guarantee modularity if the readouts are orthogonal. Consider a nonlinear representation of two scalar, bounded variables $x(t)$ and $y(t)$:
\begin{equation}
    \vg(t) = \vu(x(t)) + \vv(y(t)) + \vb
\end{equation}
Where we have, without loss of generality, made $\vu(x(t))$ and $\vv(y(t))$ mean-zero and shifted the constant component into the bias vector $\vb$. Then there is some affine readout to labels:
\begin{equation}
    \mW_{\text{out}} \cdot \vg + \vb_{\text{out}} = \begin{bmatrix}
        \vt_x(x(t)) \\
        \vt_y(y(t))
    \end{bmatrix}
\end{equation}
Again we consider an energy loss:
\begin{equation}
    \mathcal{L} = \langle |\vg(t)|^2 \rangle_t + \lambda |\mW_{\text{out}}|_F^2
\end{equation}
The nonlinear encoding functions, $\vu$ and $\vv$, must be chosen so that the labels are linearly related to the representation. Beyond that they are chosen to ensure the representation is non-negative, and the energy is minimised. We can use our previous results on the readout loss \will{Point to correct multivariate readout loss derivation} to show that the readout loss is minimised by modularising the representation. We can then study the activity loss:
\begin{equation}
    \mathcal{L}_G^D = \langle |\vg(t)|^2 \rangle_t = |\vb|^2 + \langle |\vu(x(t))|^2\rangle_t + \langle |\vv(y(t))|^2\rangle_t + 2 \langle \vu(x(t))^T\vv(y(t))\rangle_t
\end{equation}
And the minimal bias is: $\vb = -\min_t \vu(x(t)) + \vv(y(t))$.

Compare this to the modularised representation:
\begin{equation}
    \vg(t) = \begin{bmatrix}
        \vu(x(t)) \\
        \vv(y(t))
    \end{bmatrix} + \begin{bmatrix}
        \vb_x \\
        \vb_y
    \end{bmatrix}
\end{equation}
Where $\vb_x = -\min_t \vu(x(t))$ and $\vb_y = -\min_t\vv(y(t))$. Whose activity loss is:
\begin{equation}
    \mathcal{L}_G^M = |\vb_x|^2  + |\vb_y|^2+ \langle |\vu(x(t))|^2\rangle_t + \langle |\vv(y(t))|^2\rangle_t
\end{equation}
Now, if the two variables are independent from one another the modularisation result is easy. The bias must be the sum of the two constituent biases: $\vb = -\min_t \vu(x(t)) + \vv(y(t)) = -\min_t \vu(x(t)) - \min_t \vv(y(t)) = \vb_x + \vb_y$. Further, the term $\langle \vu(x(t))^T\vv(y(t))\rangle_t = 0$. Therefore:
\begin{equation}
    \mathcal{L}_G^D - \mathcal{L}_G^M = 2\vb_x^T\vb_y \geq 0
\end{equation}
And the modular solution is always better.

\subsection{Range Independent Variables Don't Always Modularise}

We call two variables range independent if knowing the value of one variable tells you nothing about the possible values of the other. This is a looser constraint than independence, as knowing the value of one variable can tell you something about the probability of another variable taking particular values, but not that it won't take any particular value. If two variables are range independent then $\min_t \vu(x(t)) + \vv(y(t)) = \min_t \vu(x(t) + \min_t\vv(y(t))$. It is like the nonlinear analogue of extreme point independence.

If two variables are range independent:
\begin{equation}
    \mathcal{L}_G^D - \mathcal{L}_G^M = 2\vb_x^T\vb_y - 2\langle \vu(x(t))^T\vv(y(t))\rangle_t
\end{equation}
Further, if the encodings are symmetrically bounded ($|\min_t \vu(x(t))| = \max_t \vu(x(t))$) then, by similar arguments to section~\ref{sec:correlated_variables}, the covariances of the encoding functions are bounded:
\begin{equation}
    \langle \vu(x(t))^T\vv(y(t))\rangle_t < \vb_x^T \vb_y
\end{equation}
Hence, symmetrically bounded encodings of range independent variables that are orthogonally decoded should always modularise. This is a lot less interpretable than its linear equivalent, however, as it relies on the bounding-symmetry of encoding functions. For non-symmetrically bounded encodings the correlations can be arbitrarily large and can lead to it being optimal to break modularity.

In general, all these encodings could point in the opposite direction, so all four quadrants are separately explored. If either of the quandrants in which the encodings align (either $x>0$ and $y>0$, or $x<0$ and $y<0$) are negative it should mix. Similarly in the other two quadrants if the value if positive they should mix.

==> Old_Writing/WeightSimilarityAttempt.tex <==

\subsection{Convex Reformulation and Global Optimality}\label{app:convex_reformulation}

We have derived conditions under which a modular solution is a local optima. In this section we show that we can rewrite the entire problem as a convex optimisation problem. We use this to show that if the modular solution is a local optima, it is also a global optima.

We're going to write the entire optimisation problem in terms of the input transformation similarity matrix. Create the following convenient variables:
\begin{equation}
    \mS' = \begin{bmatrix}
            \mS \\
            {\bf 1}
        \end{bmatrix} \qquad \mW_{\text{in}}' = \begin{bmatrix}
            \mW_{\text{in}}\mA & \vb_{\text{in}}
        \end{bmatrix} \quad \text{such that} \quad \mZ = \mW'_{\text{in}}\mS'
\end{equation}
Then the input transformation similarity matrix is $\mQ = (\mW_{\text{in}}')^T\mW_{\text{in}}'$. In order to show the problem is convex with respect to this variable we need to first show that the feasible set of allowed $\mQ$ matrices is a convex set, and second show that the objective function is a convex function of $\mQ$. We will do each of these in turn.

\subsubsection{Convex Feasible Set}

The representation has to obey three constraints:
\begin{enumerate}
    \item It has to be positive $\mZ \geq {\bf 0}$
    \item It has to be an affine function of the inputs $\mZ = \mW'_{\text{in}}\mS'$
    \item An affine map has to relate the representation back to the inputs: $\mX = \mW_{\text{out}}\mZ + \vb_{\text{out}}{\bf 1}^T$. If the matrix, $\mW_{\text{in}}'$, has full column rank, such a readout affine map will always exist.
\end{enumerate}

We now show that set of $\mQ$ matrices that create representations that satisfy each of these constraints form a convex set. Since the intersection of many convex sets is itself a convex set \citep{boyd2004convex}, this suffices to show that the set of feasible dot product matrices is convex. 

\paragraph{Affine Input and Readout} If the matrix $\mW_{\text{in}}'$ has full column rank then the data can be perfectly decoded from the representation using such an affine transformation, satisfying point 3. Further, point 2 is trivially satisfied. We now show that the convex combination of two input transformation similarity matrices that satisfy this constraint also satisfies this constraint, since they correspond to the set of positive-definite full rank matrices, which is a convex set.

Take two such matrices, $\mQ = (\mW_{\text{in}}')^T\mW_{\text{in}}'$ and $\tilde{\mQ} = (\tilde{\mW_{\text{in}}}')^T\tilde{\mW_{\text{in}}}'$. These are both positive-definite full rank matrices. Their convex combination is:
\begin{equation}
    \lambda\mQ + (1-\lambda)\tilde{\mQ} = \lambda\mW_{\text{in}}^{'T}\mW_{\text{in}}' + (1+\lambda)\tilde{\mW}_{\text{in}}^{'T}\tilde{\mW}_{\text{in}}' \quad \lambda \in [0, 1]
\end{equation}
Convex combinations of positive definite symmetric matrices are also positive definite symmetric matrices. Hence, $\lambda\mQ + (1-\lambda)\tilde{\mQ}$ can be written in terms of a unique square root: $\hat{\mW}_{\text{in}}^{'T}\hat{\mW}_{\text{in}}^{'}$ for some matrix $\hat{\mW}_{\text{in}}'$ with full column rank $d_s$. Hence both constraints 2 and 3 are satisfied.

\paragraph{Positive Representations} Take two input transformations, $\mW_{\text{in}}'$ and $\tilde{\mW}_{\text{in}}'$, such that $\mZ = \mW_{\text{in}}'\mS' \geq 0$ and $\tilde{\mZ} = \tilde{\mW_{\text{in}}}'\mS' \geq 0$. Then the representational similarity matrices $\mZ^T\mZ$ and $\tilde{\mZ^T}\tilde{\mZ}$ form a convex set, called the set of completely positive matrices \citep{sengupta2018manifold, berman2003completely}. As such, $\lambda\mZ^T\mZ$

==> iclr_2025/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

%%%%%%%%%%%%%%%% custom %%%%%%%%%%%%%%%%
\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}
\DeclarePairedDelimiterX{\infdivx}[2]{(}{)}{%
  #1\;\delimsize\|\;#2%
}
\newcommand{\infdiv}{D\infdivx}
\renewcommand{\KL}{D_\text{KL} \infdivx}
